So You Want to Analyze Scheme Programs With Datalog?

Static analysis approximates the results of a program by examining only its syntax. For example, control-flow analysis (CFA) determines which syntactic lambdas (for functional languages) or (for object-oriented) methods may be invoked at each call site within a program. Rich theoretical results exist studying control flow analysis for Scheme-like languages, but implementations are often complex and specialized. By contrast, object-oriented languages (Java in particular) enjoy high-precision control-flow analyses that scale to thousands (or more) of lines of code. State-of-the-art implementations (such as DOOP on Souffl\'e) structure the analysis using Horn-SAT (Datalog) to enable compilation of the analysis to efficient implementations such as high-performance relational algebra kernels. In this paper, we present an implementation of control-flow analysis for a significant subset of Scheme (including set!, call/cc, and primitive operations) using the Souffl\'e Datalog engine. We present an evaluation on a worst-case term demonstrating the polynomial complexity of our m-CFA and remark upon scalability results using Souffl\'e.

==> Makefile <==
PACKAGE=paper

PDF = $(PACKAGE).pdf

all:  ${PDF}

%.pdf: *.tex
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

clean:
	$(RM)  *.pdf *.aux *.log *#* *~*

.PHONY: all docclean clean archive zip


==> sec6-related.tex <==
\section{Related Work}
\label{sec:related}

Doop!

